Model Selection with Low Complexity Priors

Regularization plays a pivotal role when facing the challenge of solving ill-posed inverse problems, where the number of observations is smaller than the ambient dimension of the object to be estimated. A line of recent work has studied regularization models with various types of low-dimensional structures. In such settings, the general approach is to solve a regularized optimization problem, which combines a data fidelity term and some regularization penalty that promotes the assumed low-dimensional/simple structure. This paper provides a general framework to capture this low-dimensional structure through what we coin partly smooth functions relative to a linear manifold. These are convex, non-negative, closed and finite-valued functions that will promote objects living on low-dimensional subspaces. This class of regularizers encompasses many popular examples such as the L1 norm, L1-L2 norm (group sparsity), as well as several others including the Linfty norm. We also show that the set of partly smooth functions relative to a linear manifold is closed under addition and pre-composition by a linear operator, which allows to cover mixed regularization, and the so-called analysis-type priors (e.g. total variation, fused Lasso, finite-valued polyhedral gauges). Our main result presents a unified sharp analysis of exact and robust recovery of the low-dimensional subspace model associated to the object to recover from partial measurements. This analysis is illustrated on a number of special and previously studied cases, and on an analysis of the performance of Linfty regularization in a compressed sensing scenario.

==> sections/examples/ex-nuclear.tex <==
\subsection{Nuclear Norm Regularization}
\label{sec:ex-nuclear}

%%% OLD, not used %%%

The nuclear norm, or trace norm, has been proposed as an effective convex relaxation for rank minimization problems to provably recover low-rank matrices \cite{candes2009exact,recht2010guaranteed}.
The nuclear norm of a $N_1 \times N_2$ rank-$r$ matrix x is defined as $\J(x) = \norm{x}_* = \norm{\diag(\Sigma)}_1$, where $x=U \Sigma V^*$ is a reduced singular value decomposition (SVD) of $x$, with $\diag(\Sigma)=(\sigma_i)_{1 \leq i \leq r}$ the singular values, $U$ ($N_1 \times r$) and $V$ ($N_2 \times r$) are the matrices of left and right singular vectors.

%%%%
\subsubsection{Structure of the nuclear norm}

In the following, we show that the nuclear norm is a symmetric strongly piecewise regular gauge.
\begin{prop}\label{prop:ex-nuclear-swdg}
  The nuclear norm is a symmetric strong gauge with
  \begin{gather*}
    \S_x = \enscond{ U_\bot^* C V_\bot }{  C \in \RR^{(N_1-r) \times (N_2-r)} }, \\
    \T_x = \enscond{ U A^*  + B V^* }{ A \in \RR^{N_2 \times r}, B \in \RR^{N_1 \times r}}
          = \enscond{Z \in \RR^{(N_1-r) \times (N_2-r)}}{ U_\bot^* Z V_\bot = 0 }, \\
    \e_x = U V^*, \quad
    \f_x = \e_x, \quad
    \Js(x) = \umax{i} \sigma_i + \iota_{\S_x} ~,
  \end{gather*}
  where $U_\bot,V_\bot$ span the orthogonal of the ranges of $U,V$.
  Moreover, it is strongly piecewise regular with parameters
  \begin{equation*}
    \nu_x = \frac{1}{4} \umin{i \in I} |\sigma_i| ,
    \quad
    \mu_x = \frac{1}{\nu_x}
    \qandq
    \tau_x = \xi_x = 0 .
  \end{equation*}
\end{prop}
I can be observed that $\dim(\T_x)=r(N_1+N_2-r)$ and $\dim(\S_x)=N_1N_2-\dim(\T_x)=N_1N_2-r(N_1+N_2)+r^2$.

%%%%
\subsubsection{Relation to previous work}

The work in~\cite{bach2008trace} defines an irrepresentabilty condition for the nuclear norm. 
This irrepresentability condition is assumed in~\cite{bach2008trace} to establish asymptotic rank consistency of nuclear norm minimization in the overdetermined case.
Similarly to \eqref{eq-block-irrepres}, this condition can be shown to be equivalent to our condition $\IC(x_0)<1$, when specialized to the case of the nuclear norm. Note also that \cite{bach2008trace} provides a proof of the PRG property of the nuclear norm (Proposition~\ref{prop:ex-nuclear-swdg}).  In their unified framework, the work~\cite{recht2010guaranteed} derives tight bounds on the number of Gaussian measurements needed for exact and robust recovery by nuclear norm minimization. The work of~\cite{recht2010guaranteed} complements these results, using the irrepresentable condition tailored to the nuclear norm, to get tight bounds for noiseless identifiability. 


Let us also point out that the recent work of \cite{grave2011trace} considers an analysis-type form of the nuclear norm, the so-called trace Lasso. However no recovery guarantees (with or without noise) were given. In fact, combining Proposition~\ref{prop:ex-nuclear-swdg} and the results on the pre-composition rule given in Section~\ref{sec:alge-precomp}, one can establish piecewise regularity and derive theoretical recovery guarantees for the trace Lasso.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../robust-convex-regularization"
%%% End: 


==> sections/proofs/proofs-polar.tex <==
% !TEX root = ../../IMAIAI-PartlySmoothLinear.tex


\section{Results on the Polar Set and Gauge}

Similarly to the duality inequality for norms, a gauge and its polar satisfies some kind of Holder inequality as stated below.
\begin{lem}[Holder Inequality]\label{lem:convex-holder}
  Let $\gauge$ be a gauge on $\RR^N$.
  Then
  \begin{equation*}
    \foralls (x,x^\circ) \in \dom \gauge \times \dom \gauge^\circ, \quad
    \dotp{x}{x^\circ} \leq \gauge(x) \gauge^\circ(x^\circ) .
  \end{equation*}
\end{lem}

Throughout, we will consider only closed convex subsets of $\RR^n$ containing the origin. For a subset $C$ of $\RR^n$, we say that the subsets defined by
\begin{align*}
C^\circ &= \enscond{u \in \RR^n}{\dotp{x}{u} \leq 1, \quad \forall x \in C} \\
C^- &= \enscond{u \in \RR^n}{\dotp{x}{u} \leq 0, \quad \forall x \in C} \\
C^\perp &= \enscond{u \in \RR^n}{\dotp{x}{u} = 0, \quad \forall x \in C} ~.
\end{align*}
are the polar set, the (negative) polar cone and the orthogonal space of $C$ respectively. We denote $\cl{\cdot}$ the closure and $\co{\cdot}$ the (closed) convex hull.

We now collect important results on polar calculus some of which are well-known (see e.g. \cite[Chapters 14-16]{rockafellar1996convex}, Zalinescu Chapter 1, Borwein-Lewis Chapter 4).
\begin{lem}
\label{lem:polarsets}1
{~}\vskip 1pt
\begin{enumerate}
\item $C^\circ$ is closed convex containing the origin (even if $0 \notin C$), $C^-$ is a closed convex cone, and $C^\perp$ is a closed linear subspace.
\item Bipolar: $C^{\circ\circ}=C$ (otherwise, in general $C^{\circ\circ}=\co{C \cup \{0\}}$).
\item Reverse ordering: $C \subset D \Rightarrow D^\circ \subset C^\circ$.
\item $(C \cup D)^\circ=C^\circ \cap D^\circ$.
\item $(C \cap D)^\circ=\co{C^\circ \cup D^\circ}$.
\item $(\rho C)^\circ = C^\circ/\rho$, $\forall 0 < \rho < \infty$.
\item $(C+D)^-=(C \cup D)^-=C^- \cap D^-$.
\item If $C$ is a cone, $C^\circ=C^-$.
\item If $C$ is a linear subspace, $C^\circ=C^-=C^\perp$.
\item If $C$ and $D$ are cones, then $(C+D)^\circ=(C \cup D)^\circ=C^\circ \cap D^\circ$.
\item If $C$ is a cone and $D$ is a closed convex subset containing the origin, then $(C + D)^\circ=C^\circ \cap D^\circ$.
\end{enumerate}
\end{lem}

The proof of the last item is the less straightforward. It can be obtained as follows. First, one can observe that for two convex sets
\[
\co{C \cup D} = \bigcup_{\rho \in [0,1]} \rho C + (1-\rho) D ~.
\]
Thus, we get
\begin{align*}
(C \cap D)^\circ	&= \co{C^\circ \cup D^\circ} \\
				&= \bigcup_{\rho \in [0,1]} \rho C^\circ + (1-\rho) D^\circ \\
				&= \bigcup_{\rho \in [0,1]} C^\circ + \rho D^\circ \\
				&= C^\circ+D^\circ ~,
\end{align*}
where we used $(v)$, $(ii)$, that $C$ is a cone and both sets are closed convex and contain the origin.

We recall that a fundamental result of convex analysis states that there is a one-to-one correspondence between closed sublinear functions and closed convex sets. This allows to identify sets from their support functions or from their polar gauges, and vice versa. We denote in the sequel $\sigma_C$ and $\gamma_C$ the support and the gauge of $C$. We also recall that $\sigma_C$ and $\gamma_C$ are polar to each other, i.e. $\gamma_C=\sigma_{C^\circ}$.

\begin{prop}
\label{prop:gaugesum}
Let $C=C_1+C_2$, where $C_1$ and $C_2$ are nonempty closed convex sets containing the origin. Assume in addition that their relative interiors intersect and that their Minkowski sum is closed. For some $0 < \rho < \infty$, the identity 
\[
\gamma_C = \rho \gamma_{C_1} \infc \gamma_{C_2} 
\]
is equivalent to
\[
C_1+C_2=\rho^{-1}\co{C_1 \cup C_2} ~.
\]
\end{prop}

\begin{proof}
Since all sets are closed convex and contain the origin, we have
\begin{align*}
\gamma_C	&= \gamma_{C_1+C_2} = \sigma_{(C_1+C_2)^o} \\
			&= \rho \sigma_{C_1^\circ \cap C_2^\circ} = \rho \sigma_{C_1^\circ} \infc \sigma_{C_2^\circ} = \rho \gamma_{C_1} \infc \gamma_{C_2} \\
			&= \rho \sigma_{(C_1 \cup C_2)^\circ} = \sigma_{((C_1 \cup C_2)/\rho)^\circ} ~.
\end{align*}
where we used Lemma~\ref{lem:polarsets}$~(v)$-$(vi)$. Note that the qualification condition on the relative interiors is important for the fourth equality to hold. Thus, by uniqueness of the sets and bipolarity, we get $C_1+C_2 = ((C_1 \cup C_2)/\rho)^{\circ\circ}=\rho^{-1}\co{C_1 \cup C_2}$.
\end{proof}

%%%%
\subsubsection{Examples}

\begin{itemize}
	\item If $C_1=C_2$, then the proposition holds with $\rho=1/2$. Indeed $C_1+C_2=2C_1=2(C_1 \cup C_2)$.
	\item If $C_1$ and $C_2$ are cones, the proposition holds with $\rho=1$. Another way of seeing it is from Lemma~\ref{lem:polarsets}~$(x)$.
\end{itemize}

What can be said in general if neither $C_1$ nor $C_2$ is a cone for Lemma~\ref{lem:polarsets}~$(x)$ or $(xi)$ to apply. One can observe that depending on the structure of the Minkowski sum with respect to the convex hull of the union, one can upper or a lower bound the gauge of one with that of the other (using the fact that the gauge reverses the ordering of sets). We can however prove the following result. For this, we introduce the inverse sum of two sets (or convolution of the sets since they are convex) :
\[
	C_1 \otimes C_2 = \cl{\bigcup_{\rho \in [0,1]} \rho C \cap (1-\rho) D} ~.
\]

\begin{prop}
\label{prop:polarsum}
Let $C_1$ and $C_2$ be nonempty closed convex sets containing the origin. Then
\[
	(C_1+C_2)^\circ = C_1^\circ \otimes C_2^\circ ~.
\]
Therefore
\[
	\gamma_{C_1+C_2} = \sup_{\rho \in [0,1]} \rho\gamma_{C_1} \infc (1-\rho)\gamma_{C_2} ~.
\]
\end{prop}

\begin{proof}
From Demyanov and Rubinov, Chapter~3, Remark 7.1, we know that
\[
\gamma_{C_1 \otimes C_2} = \gamma_{C_1} + \gamma_{C_2} ~.
\]
Hence,
\begin{align*}
\gamma_{C_1 \otimes C_2}	&= \sigma_{(C_1 \otimes C_2)^\circ} \\
						&= \sigma_{C_1^\circ} + \sigma_{C_2^\circ} \\
						&= \sigma_{C_1^\circ+C_2^\circ} ~,
\end{align*}
which by bipolarity and uniqueness of the sets in the correspondence, yields
\[
(C_1+C_2)^\circ = \co{C_1^\circ \otimes C_2^\circ} = C_1^\circ \otimes C_2^\circ ~.
\]
We now have
\begin{align*}
\gamma_{C_1+C_2}(x)	&= \sigma_{C_1^\circ \otimes C_2^\circ}(x) \\
					&= \sup_{u \in C_1^\circ \otimes C_2^\circ} \dotp{x}{u} \\
					&= \sup_{\rho \in [0,1]} \sup_{u \in \rho C_1^\circ \cap (1-\rho)C_2^\circ} \dotp{x}{u} \\
					&= \sup_{\rho \in [0,1]} \sigma_{\rho C_1^\circ} \infc \sigma_{(1-\rho) C_2^\circ}(x) \\
					&= \sup_{\rho \in [0,1]} \rho\sigma_{C_1^\circ} \infc (1-\rho)\sigma_{C_2^\circ}(x) \\
					&= \sup_{\rho \in [0,1]} \rho\gamma_{C_1} \infc (1-\rho)\gamma_{C_2}(x) ~,
\end{align*}
where we used that $\rho C_1^\circ \cap (1-\rho)C_2^\circ \neq \emptyset$ for any $\rho \in [0,1]$.
\end{proof}
One can easily verify that we recover the results of Lemma~\ref{lem:polarsets}~$(x)$ and $(xi)$ as well as the first example above in the corresponding special cases. 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../robust-convex-regularization"
%%% End: 

